Orbital Optimization in the Density Matrix Renormalization Group, with applications to polyenes and \beta-carotene

In previous work we have shown that the Density Matrix Renormalization Group (DMRG) enables near-exact calculations in active spaces much larger than are possible with traditional Complete Active Space algorithms. Here, we implement orbital optimisation with the Density Matrix Renormalization Group to further allow the self-consistent improvement of the active orbitals, as is done in the Complete Active Space Self-Consistent Field (CASSCF) method. We use our resulting DMRGCASSCF method to study the low-lying excited states of the all-trans polyenes up to C24H26 as well as \beta-carotene, correlating with near-exact accuracy the optimised complete \pi-valence space with up to 24 active electrons and orbitals, and analyse our results in the light of the recent discovery from Resonance Raman experiments of new optically dark states in the spectrum.

==> density.tex <==
% \input{header.tex}

% \begin{document}

In the one-site DMRG ansatz, when we are in the canonical
representation of site $p$ (i.e. the block configuration where the left
block spans sites $1 \ldots p-1$, and the right block, sites $p+1
\ldots k$), we are working with the renormalised product space 
$\{l_{p-1}\} \otimes \{ n_p \} \otimes \{ r_{p+1} \}$. Thus we need
matrix representations of operators in each of the three spaces,
i.e. matrix elements $\langle {l^{p-1}} | \hat{O} |
{l^{p-1}}^\prime \rangle$, $\langle n^{p} | \hat{O} |
{n^{p}}^\prime \rangle$, $\langle r^{p+1} | \hat{O} |
{r^{p+1}}^\prime \rangle$.
Matrix representations  in the left and right subspaces are in general of dimension $O(M\times M)$.
To solve the Schr\"odinger equation, we need the action of the
Hamiltonian,  $\hat{H} |\Psi\rangle$ which would  appear to require
storage of ${O(k^4)}$ operators  $a^\dag_i a^\dag_j a_k
a_l$ with a concomittant memory cost of $O(M^2 k^4)$.
However, the memory cost of the standard quantum chemical DMRG
algorithm is only $O(M^2 k^2)$. This is because 
we do not actually need the action of the operators $a^\dag_i a^\dag_j a_k a_l$ individually, but only the
sum $\sum_{ijkl} v_{ijkl} a^\dag_i a^\dag_j a_k a_l$, and thus we can
manipulate groupings of operators that are precontracted with two-electron
integrals to save memory. For example, the sum of operators in the Hamiltonian may be written in
the form (considering the single site $p$  to be part of the left
block for simplicity) 
\begin{align}
\hat{H} &= \sum_{ij} t_{ij} a^\dag_i a_j + \sum_{ijkl} v_{ijkl} a^\dag_i
a^\dag_j a_k a_l \nonumber\\
  &= \hat{H}^L + \hat{H}^R + \sum_{i \in L} a^\dag_i S_i + c.c. + \sum_{ij \in L} a^\dag_i
  a^\dag_j P_{ij}^R + a^\dag_i a_j Q_{ij}^R \label{eq:h_eq}
\end{align}
where
\begin{align}
\hat{H}^L & = \sum_{ij \in L} t_{ij} a^\dag_i a_j + \sum_{ijkl \in L} v_{ijkl} a^\dag_i
a^\dag_j a_k a_l \nonumber \\
\hat{H}^L & = \sum_{ij \in R} t_{ij} a^\dag_i a_j + \sum_{ijkl \in R} v_{ijkl} a^\dag_i
a^\dag_j a_k a_l \nonumber \\
\hat{S}_i &= \sum_{j \in R} t_{ij}  a_j + \sum_{jkl \in R} (v_{ijkl} -
v_{jilk}) a^\dag_j a_k a_l \nonumber \\
\hat{P}_{ij}^R &= \sum_{kl \in R} v_{ijkl} a_k a_l \nonumber \\
\hat{Q}_{ij}^R &= \sum_{kl \in R} (v_{ijkl} - v_{jikl} - v_{ijlk} + v_{jilk}) a^\dag_k a_l 
\end{align}
In the form (\ref{eq:h_eq}) the  intermediates appearing  e.g. $\hat{P}_{ij}^R, \hat{Q}_{ij}^R$ carry at
most two orbital indices, and so we can evaluate $\hat{H}|\Psi\rangle$ at any block configuration
by manipulating only $O(k^2)$ operator matrices,  which leads to the
$O(M^2 k^2)$  memory cost of the quantum chemical DMRG algorithm.  


% We have implemented the above algorithm for the determination of the
% two-particle density matrix in our code Block. The overall
% computational cost per sweep is $O(M^3 k^4)$, the memory per block
% iteration is $O(M^2 k^2)$, where $k$ is the size of the active space
% and $M$ is the number of DMRG states. In addition our
% algorithm is automatically parallelised because of our strategy of
% distributing operators across processors as described in Ref. X. Thus,
% the parallel cost of our algorithm is X.

% [Then some stuff on parallel evaluation]


%\end{document}

